Exploring Linkablility of Community Reviewing

Large numbers of people all over the world read and contribute to various review sites. Many contributors are understandably concerned about privacy; specifically, about linkability of reviews (and accounts) across review sites. In this paper, we study linkability of community reviewing and try to answer the question: to what extent are "anonymous" reviews linkable, i.e., likely authored by the same contributor? Based on a very large set of reviews from a popular site (Yelp), we show that a high percentage of ostensibly anonymous reviews can be linked with very high confidence. This is despite the fact that we use very simple models and equally simple features set. Our study suggests that contributors reliably expose their identities in reviews. This has important implications for cross-referencing accounts between different review sites. Also, techniques used in our study could be adopted by review sites to give contributors feedback about privacy of their reviews.

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}
%
As mentioned in Section \ref{sec:background}, we use Na\"ive Bayes (NB) and 
Kullback-Leibler Divergence (KLD) models.
Before analyzing the collected data, we tokenize all reviews. From each review, we extract three types of tokens:
%
\begin{enumerate}
%
\item \textbf{Unigrams:} set of all single letters. We discard all non-alphabetical characters.
%
\item \textbf{Digrams:} set of all consecutive letter-pairs. We discard all non-alphabetical characters. 
%
\item \textbf{Rating:} rating associated with the review. (In Yelp, it ranges between 1 and 5).
%
\end{enumerate}
%
\noindent{\bf Why such simple tokens?} Our choice of these three primitive token types might
seem trivial or even na\"ive. In fact, initial goals of this study included more ``sophisticated''
types of tokens, such as: (1) distribution of word usage, (2) sentence length in words, and (3) punctuation
usage. We originally planned to use unigrams and digrams as a baseline, imagining that (as long as all 
reviews are written in the same language -- English, in our case) single and double-letter
distributions would remain more-or-less constant across contributors. However, as our results
clearly indicate, our hypothesis was completely wrong. 

In the rest of this section, we analyze results produced by NB and KLD models.
% From here on, the term "token" refers to unigram, digram or rating. 
Before proceeding, we re-cap abbreviations and our notation in Table \ref{tab:notation}.
%
\begin{table}[t!]
\begin{center}
\begin{tabular}{|r|l|}
\hline
NB  & Na\"ive Bayes Model 
\\ \hline
KLD  & Symmetrical Kullback-Leibler Divergence Model
\\  \hline 
R  & Token Type: rating, unigram or digram
\\ \hline
LR & Linkability Ratio
\\ \hline
AR & Anonymous Record 
\\ \hline 
IR  & Identified Record (corresponding to a certain reviewer/account) 
\\ \hline
$SymD_{KLD}(IR,AR)$  & symmetric KLD distance between $IR$ and $AR$
\\ \hline
\end{tabular}
\end{center}
\caption{Notation and abbreviations.}
\label{tab:notation}
\end{table}%


\subsection{Methodology}
\label{method}
We begin with the brief description of the methodology for the two models.


\subsubsection{Na\"ive Bayes (NB) Model}
\label{sec:nb-method}
%
For each account $IR$, we build an NB model, $P(token_i|IR)$,  from its identified record. Probabilities are computed using the Maximum-Likelihood estimator \cite{bishopbook} and Laplace smoothing \cite{mlearn1} as shown in \ref{sec:background}. We then construct three models corresponding to the three aforementioned token types.
That is, for each $IR$, we have $P_{unigram}$, $P_{digram}$, and $P_{rating}$.

\if 0
\[P(token_i|IR)=\frac{Num\ of\ Occurrences\ of\ Token_i}{Num\ of\ Occurrences\ of\ all\ Tokens}\]
 
We smooth the probabilities with Laplace smoothing \cite{mlearn1} as follows:
\[P(token_i|IR)=\frac{Num\ of\ Occurrences\ of\ Token_i\ +\ 1}{Num\ of\ Occurrences\ of\ all\ Tokens\ +\ Num\ of\ Possible\ Token\ Values}\]
 
We then construct three models corresponding to the three aforementioned token types. 
That is, for each $IR$, we have $P_{unigram}$, $P_{digram}$, and $P_{rating}$.
\fi
To link an anonymous record $AR$ to an account $IR$ with respect to token type $R$, we first extract 
all $R$-type tokens from $AR$, $T_{R_1}, T_{R_2}, ....T_{R_n}$ (Where $T_{R_i}$ is the $i$-th 
$R$ token in $AR$). 
%
%GTS: What is UIT_{R_1} --- not defined!!!
Then, for each $IR$, we compute the probability $P_R(IR|T_{R_1}, T_{R_2}, ....T_{R_n})$.
Finally, we return a list of accounts sorted in decreasing order of probabilities. The top entry represents 
the most probable match.  

\subsubsection{Kullback-Leibler Divergence (KLD) Model}
\label{sec:kl-method}
%
We use symmetric KLD (see Section \ref{sec:background}) to compute the distance between 
anonymous and identified records. To do so, we first compute distributions of all records, as follows:
%
\[ 
Dist\_token(Token_i) = \frac{Num\ of\ Occurrences\ of\ Token_i}{Num\ of\ Occurrences\ of\ all\ Tokens}
\]
To avoid division by 0, we smooth distributions via Laplace smoothing \cite{mlearn1}, as follows:
\[ 
Dist\_token(Token_i) = \frac{Num\ of\ Occurrences\ of\ Token_i\ +\ 1}
{Num\ of\ Occurrences\ of\ all\ Tokens\ +\ Num\ of\ Possible\ Token\ Values}\]
%
As before, we compute 
three distributions for: rating, unigram, and digram.
To link $AR$ with respect to token type $R$, we compute $SymD_{kl}$ between the distribution of
$R$ for  $AR$ and the distribution of $R$ for each $IR$. Then, we return a list sorted in
ascending order of $SymD_{KLD}(IR,AR)$ values. The first entry represents the account with the most likely
match.


\subsection{Study Results}
\label{sec:results}
%
We now present the results, starting with those for each of the three tokens: rating, unigram and digrams.
In the following section, we experiment with certain combinations thereof.

\subsubsection{Rating}
\label{sec:rating-results}
\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:rate-nb-1-165}\includegraphics[scale=0.6]{figures/rate-nb-1-165.eps}}
  \subfigure[]{\label{fig:rate-kl-1-165}\includegraphics[scale=0.6]{figures/rate-kl-1-165.eps}}
  \caption{LRs for NB and KLD models rating tokens}
  \label{fig:rating-1-165}
\end{figure}
%
Figures \ref{fig:rate-nb-1-165} and \ref{fig:rate-kl-1-165} show linkability ratios (LRs) for NB and KLD models, respectively,  
for several anonymous record sizes when rating alone is used as the token. Top-1, Top-10, and Top-50 plots are shown 
in both figures. Not surprisingly, an increase in the anonymous record size causes an increase in LR. In the Top-1 plot,
LR is low and the highest ratio is 1.5\%/2\% in NB/KLD when anonymous record size is 165. However, in Top-10 and 
Top-50 plots, LRs become higher. For example, for record size of 165, LRs are around 9\% and 26\% for Top-10 and 
Top-50 plots, respectively, in both models. 
%
%GTS: this sentence makes no sense at all.
%In addition, for the Top-500 (top 25\%) linkability ratio (not shown in the figure) in NB/KLD model, 
% the ratio is 55.9\%/49.9\% when record size is 10,  67.4\%/65.6\% when 
% record size is 30\% and over 70\%/70\% when record size is over 30. 
We thus conclude that this model is somewhat helpful but, by itself, insufficient to link accounts for many 
anonymous records. However, it turns out to be very useful when combined with other lexical tokens,  
as discussed in Section \ref{sec:combine-model} below. We observe that the performance of the two 
models  is comparable. 


\subsubsection{Unigram}
\label{sec:unigram-results}
%
\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:ng-1-nb-1-165}\includegraphics[scale=0.6]{figures/text_ng_1_nb-1-165.eps}}
  \subfigure[]{\label{fig:ng-1-kl-1-165}\includegraphics[scale=0.6]{figures/text_ng_1_kl-1-165.eps}}
  \caption{LRs of NB and KLD models for unigram tokens}
  \label{fig:unigram-1-165}
\end{figure}
%
Figures \ref{fig:ng-1-nb-1-165} and \ref{fig:ng-1-kl-1-165} 
show LRs (Top-1 and Top-10) for NB and KLD with the unigram token. 
As expected, with an increase in anonymous record size, LR grows: it is high in both Top-1 and Top-10 plots. 
For example, in Top-1 of both figures, LRs are around: 36.5\%, 59\% and 66\% for anonymous record sizes of 30, 80 and 165, 
respectively.  Whereas, in Top-10 of both figures, LRs are around: 66.5\%, 83\% and  86.5\% for same record sizes. 
This suggests that reviews are highly linkable based on trivial single-letter distributions. Note 
that the two models exhibit similar performance.  


\subsubsection{Digram}
\label{sec:digram-results}
%
\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:ng-2-nb-1-165}\includegraphics[scale=0.6]{figures/text_ng_2_nb-1-165.eps}}
  \subfigure[]{\label{fig:ng-2-kl-1-165}\includegraphics[scale=0.6]{figures/text_ng_2_kl-1-165.eps}}
  \label{fig:digram-1-165}  
  \caption{LRs of NB and KLD models for digram tokens}
\end{figure}
%
Figures \ref{fig:ng-2-nb-1-165} and \ref{fig:ng-2-kl-1-165} consider the digram token.
In both models, LR is impressive in both plots: it gets as high as 95.8\%/98.3\% in Top-1 and 
98.4\%/99.2\% in Top-10 plot for NB/KLD, respectively.  It appears that, so far, digrams offer the best 
(most reliable) linkability results. 

Unlike rating and unigrams -- where LRs in both models are comparable for various record sizes-- KLD  
starts with LRs considerably lower than those of  NB. However, the situation changes when record size reaches 80, 
with KLD performing better for large record sizes. One reason for this reversal  could be that KLD improves 
when the distribution of anonymous records is more similar to that of corresponding identified records; this 
usually occurs for large record sizes, as there are more tokens.      

Not surprisingly, larger record sizes entail higher LRs. With NB, larger record sizes increase the number
of tokens common to both the anonymous record and its corresponding identified one. For KLD, larger record sizes cause the distribution 
derived from the anonymous record to be more similar to the one derived from the corresponding identified record.

However, somewhat  unexpectedly, we observe that the LR in both models decreases when record 
size reaches 100/130 for NB/KLD models. One possible reason for this phenomenon is that
%, when the record size exceeds 100/130, 
some outlier tokens start to appear in some anonymous records. For NB, this may decrease probabilities for the actual 
corresponding accounts. For KLD, this may make the distribution derived from the anonymous record less similar 
to the real distribution of the actual account \footnote{For KLD, the inclusion of outlier tokens into the anonymous record could 
lead to a significant increase in these tokens probabilities in anonymous distributions since the number tokens in 
the anonymous record is way less than the number of tokens in the identified record, which used to have these 
outlier tokens with small probabilities. As a result, the distance between the identified record and its corresponding 
anonymous one increases.}.


\subsection{Improvement I: Combining Rating with Lexical Tokens}
\label{sec:combine-model}
%
In an attempt to further improve LRs, we now combine the rating token with is lexical counterparts.


\subsubsection{Combining Tokens in NB}
\label{sec:method-nb-combine}
%
This is straightforward in the NB. We simply increase the list of tokens in unigram/digram based NB 
by adding the rating tokens. Thus, for every $AR$, we have $P(lexical\_token_i|IR)$ and $P(rate\_token_i|IR)$. 


\subsubsection{Combining Tokens in KLD}
\label{sec:method-kl-combine}
%
\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:train-1-subset}\includegraphics[scale=0.6]{figures/train-subset-rate-gram-1.eps}}
  \subfigure[]{\label{fig:train-2-subset}\includegraphics[scale=0.6]{figures/train-subset-rate-gram-2.eps}}
  \caption{Results of combining unigram/digram tokens with ratings using different $\alpha$ values}
  \label{fig:train-subset}
\end{figure}

Combining rating with lexical (unigram or digram) token in KLD is less clear than in NB. 
One way is to simply average $SymD_{KLD}$ values for both token types. However, this might
degrade performance since lexical distributions convey much more information than rating;
thus, giving them the same weight would not yield better results. Instead, we combine them 
using a weighted average: 
%
\[ 
SymD_{kl\_combine}(P,Q) = \alpha \times SymD_{kl\_lexical}(P,Q) + (1 - \alpha) \times SymD_{kl\_rating}(P,Q) 
\] 
%
Intuitively, $SymD_{kl\_lexical}$ should have more weight as it carries more information. Since there is not a clear 
way of assigning $\alpha$ values, we experimented with several choices and picked the one with the best 
performance. We experimented only within the identified record set and then verified the results generalize to 
the anonymous record set. In more detail, this is done as follows: 

First, for every IR, we allocated the last 165 reviews as a testing record and the remainder -- as a training record. 
Then, we used KLD with several $\alpha$ values and assessed the resulting linkability ratio on 
testing records. We then picked the value of $\alpha$ with the highest LR based on testing records.  
Note that we could only use $795$ accounts  (out of $1,997$ total) in the training operation since that is the number of 
reviewers with identified records of size at least  $330\;(=165*2)$.
%
%GTS: don't understand this..
% Even though testing record size was fixed at 165, 
% for the purpose of validation (see below), selected $\alpha$ value on the set of anonymous records, 
% we observe improvements for the different sizes of the anonymous record.

Figure \ref{fig:train-subset} shows LR (Top-1) for $\alpha$ values ranging from $0.99$ to $1.00$ in $0.001$ increments. 
For further verification, we also experimented with smaller values: $0.0, 0.3, 0.5, 0.7,  \mbox{and}\ 0.9$,
all of which yielded
LRs significantly lower than 0.99 (in both unigram and digram). For unigrams, Figure \ref{fig:train-1-subset} shows an 
increasing trend for LR until it tops off at $79.5\%$ with $\alpha=0.997$ which is significantly higher than LR 
of $72.5\%$ when $\alpha=0.99$. After that, LR gradually decreases until $\alpha=1$, where $LR=74.5\%$. 
Thus, we selected $\alpha=0.997$ in the unigram case. In Figure \ref{fig:train-2-subset}, LRs are very close for 
$\alpha$ ranging between $0.99$ and $1.00$.  LR tops off at $\alpha$ of 0.992, 0.993 and 0.994. Since they all 
yield the same LR, we picked $\alpha=0.993$ for the digram case.



\subsubsection{Combining Unigrams with Ratings}
\label{sec-results-uni-rate-combine}
%
\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:ng-1-r-nb-1-165}\includegraphics[scale=0.6]{figures/text_ng_1_r_nb-1-165.eps}}
   \subfigure[]{\label{fig:ng-1-r-kl-1-165}\includegraphics[scale=0.6]{figures/text_ng_1_r_kl-1-165.eps}}
  \caption{LRs of NB and KLD  for combined ratings and unigrams}
  \label{fig:ng-1-r-1-165}
\end{figure}

Figures \ref{fig:ng-1-r-nb-1-165} and \ref{fig:ng-1-r-kl-1-165} show the plots before and after adding rating to 
unigram in the NB and KLD models, respectively, for various record sizes. As can be observed, adding rating 
increase LRs for all record sizes in both models. For Top-1, LR increases $\sim$  6-7\%/5-8\% for most 
record sizes in NB/KLD models. 
% For example, in the NB model the ratio increases from 36.4\% to 42.4\% when the record size is 30, from 
% 59\% to 65.3\% when the record size is 80 and from 66.3\% to 72.5\% when the record size is 165. 
% Similarly, in the KLD model, the linkability ratio increases from 36.6\% to 41.8\% when the record 
% size is 30, from 59\% to 64.2\% when the record size is 80, and from 66.4\% to 72.2\% when the record size is 165. 
%
A similar improvement applies to the Top-10 plot, for all the record sizes. However, it is smaller,
within 3-5\% range in both models. 
% For example, in NB model, it increases from 66.5\% to 71.6\% when the record size is 30, from 83\% to 
% 87.5\% when the record size is 80 and from 86.5\% to 90\% when the record size is 165. Similarly, in 
% KLD model, the ratio increases from 66.2\% to 70.3\% when the record size is 30, from 83.2\% to 87.7\% 
% when the record size is 80 and from 86.6\% to 90.7\% when the record size is 165.
%
Note that,  in KLD, we extract optimal $\alpha$ value by training and testing on a record size of 165. 
This $\alpha$ value is useful in improving LRs for all record sizes. In fact, the improvement in record 
size of 165 (5.8\%) is comparable to those for most other record sizes.  


\subsubsection{Combining Digrams with Ratings}
\label{sec-results-digram-rate-combine}
%
\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:ng-2-r-nb-1-165}\includegraphics[scale=0.6]{figures/text_ng_2_r_nb-1-165.eps}}
  \subfigure[]{\label{fig:ng-2-r-kl-1-165}\includegraphics[scale=0.6]{figures/text_ng_2_r_kl-1-165.eps}}
  \caption{LRs for NB an KLD combining ratings with digrams}
  \label{fig:ng-2-r-1-165}
\end{figure}
%
Figures \ref{fig:ng-2-r-nb-1-165} and \ref{fig:ng-2-r-kl-1-165} show the effect of adding ratings to digrams. 
The overall effect is minuscule: for Top-1 in NB, LR grows around 0.2-0.4\%, depending on the record size.
For Top-1 in KLD, LR grows model increases by $0.2-2.0\%$, depending on the record size.
Similar increases were observed for top-10 LRs in both models. Overall, most increases are small
which leads us to conclude that combining ratings with diagrams is not particularly effective.


\subsubsection{Improvement II: Matching all Anonymous Records at Once}
\label{sec:inter-model}
%
We now experiment with another natural strategy of attempting to match all anonymous records at once.

\subsubsection{Methodology}
\label{sec-method-once}
%
\begin{figure}[h]
%\begin{table}[h]
\begin{center}
\begin{tabular}{rl}
\hline\hline
\multicolumn{2}{l}{\textbf{Algorithm $Match\_All$:} Pseudo Code}\\
\hline
\textbf{Input}:& (1) Set of anonymous records: $S_{AR}=\{AR_1, AR_2, ...,AR_n\}$ \\
               & (2) Set of reviewer-ids / identified records: $S_{IR}=\{IR_1, IR_2, ..., IR_n\}$ \\
		&(3) Set of matching lists for each AR: $S_L=\{List_{AR_1}, List_{AR_2}, ...,List_{AR_n}\}$ \\
\textbf{Output}:& Matching list: $S_M=\{(IR_{i_1},AR_{j_1}),É(IR_{i_n},AR_{j_n})\}$\\
1: & set $S_M=\emptyset$\\
2: & While $|S_{AR}| \neq 0$: \\
3: & \hspace{5 mm} Find $AR_i$ with smallest $SymD_{KLD}$ value in all lists in $S_L$\\
4: & \hspace{5 mm} Get the corresponding reviewer-id $IR_j$\\
5: & \hspace{5 mm} Add $(IR_j, AR_i)$ to $S_M$\\
6: & \hspace{5 mm} Delete $AR_i$ from $S_{AR}$\\
7: & \hspace{5 mm} Delete $List_{AR_i}$ from $S_L$\\
8: & \hspace{5 mm} For each $List_t$ in $S_L$, \\
%GTS: what is L_j?
9: & \hspace{10 mm} Delete tuple containing $IR_j$ from $List_t$\\
10:& \hspace{5 mm} End For\\
11:& End While\\
\hline
\end{tabular}
%
\end{center} \small
NOTE 1: $List_{AR_i}$ in $S_L$ is a list of pairs $(IR_j, V_{ij})$ where $V_{ij}=SymD_{KLD}(IR_j, AR_i)$ 

NOTE 2: $List_{AR_i}$ is sorted in increasing order of $V_{ij}$, i.e., $IR_j$ with lowest $SymD_{KLD}(IR_j, AR_i)$ 
at the top. 
\normalsize
%
% \end{table}
\caption{\label{fig:inter-kl-alg} Pseudo-Code for matching all anonymous records at once.}
\end{figure}

In the previous section, we focused on linking one anonymous record at a time. That is, 
anonymous records are independently and incrementally linked to identified records (accounts/reviewer-ids). 
One natural direction for potential improvements is to attempt to link all anonymous records at the same time.
To this end, we construct algorithm $Match\_All()$ in Figure \ref{fig:inter-kl-alg} as an add-on to 
the KLD models suggested in previous sections.


$SymD_{KLD}(IR_j, AR_i)$ symmetrically measures the distance between their ($IR_j$'s and $AR_i$'s) distributions. 
Since every $AR$ 
%
%GTS: is this true?
maps to a distinct $IR$ ($AR_i$ maps to $IR_i$), it would seem that lower $SymD_{KLD}$ would lead to better match. 
% That is, if $SymD_{KLD}(IR_j, AR_i)$ is less than $SymD_{KLD}(IR_j, AR_l)$, it is very intuitive to 
% believe that $IR_j$ maps to $AR_i$ more than to believe it maps to $AR_l$ as $SymD_{KLD}$ 
% measures the distance between the two distributions and thus, the smaller the distance the more 
% confident we are in the mapping.   
We use this intuition to design $Match\_All()$.
%  in order to boost LRs by trusting lower $SymD_{KLD}$ values to represent better matches. 
%
As shown in the figure, $Match\_All()$ picks the smallest $SymD_{KLD}(IR_j, AR_i)$ as the map between $IR_j$ and $AR_i$ and 
then deletes the pair $(IR_j, V_{kj})$ from all remaining lists in $S_L$. The process continues until we compute all matches. 
Note that, for any $List_{AR_k}$, $(IR_j, V_{kj})$ is deleted from the list only when there is another pair $(IR_j, V_{lj})$ in 
$List_{AR_l}$, such that $SymD_{KLD}(IR_j, AR_l) \le SymD_{KLD}(IR_j, AR_k)$, and $IR_j$ has been selected as the match 
for $AR_l$.The output of the algorithm is a match-list: $S_M=\{(IR_{i_1},AR_{j_1}),É(IR_{i_n},AR_{j_n})\}$. 


We now consider how $Match\_All()$ could improve LRs. Suppose that we have two anonymous records $AR_i$ and $AR_j$ 
%
%GTS: what is L_i and L_j? You didn't define them. Do you mean List_{AR_i} and List_{AR_j}
along with their sorted lists $L_i$ and $L_j$ and assume that $IR_i$ is the top of each list.
Using only KLD, we would return $IR_i$ for both $AR$-s and thus miss one of the two.
Whereas, $Match\_All$, would assign $IR_i$ to {\bf only} one anonymous record -- the one with
the smaller $SymD_{KLD}(IR_i, ...)$ value.
%
%
%GTS: this makes no sense to meÉ
%
% Note that there is a chance that  $SymD_{KLD}(IR_i, AR_i) > SymD_{KLD}(IR_i, AR_j)$ and this will lead  to two 
% misses instead of one. Thus, the more that the inequality $SymD_{KLD}(IR_i, AR_i)\ <\ SymD_{KLD}(IR_i, AR_j)$ 
% holds, the higher chances that $Match_All()$ will give better results. 

We note that there are no guarantees that $Match\_All()$ will always work: one  mistake in early rounds  may lead to 
others in later rounds. We believe that $Match\_All()$ works better if $SymD_{KLD}(IR_i, AR_i) < SymD_{KLD}(IR_j, AR_i)$ ($j\neq~i$) 
holds most of the time. 
%
%GTS: makes no sense.
%
% The more this inequality holds more, when the anonymous record size is larger as there are more tokens to 
% capture the actual distribution. In fact, this is the case when we experiment this algorithm and when we 
% observe a gradual degradation in the performance of $Match\_All()$ when we  decrease the anonymous record size. 
%
In the next section, we show the results of $Match\_All()$ for the record size of 165. 
As the record size gets smaller, performance worsens.\footnote{We also tried $Match\_All()$ with 
the NB model and it did not improve LRs.}. 


\subsubsection{Results}
\label{sec-results-once}
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.75]{figures/inter-kl.eps}
  \caption{Effects of $Match\_All()$  on LRs: before and after plots. ($AR$ size set to $165$).}
  \label{fig:inter-kl-model}	
\end{figure}
%
Figure \ref{fig:inter-kl-model} shows the effect of $Match\_All()$ on LR when the record size is 165. LR goes up
by a respectable 5\% for unigram and combined unigram-rating models. However, for digram and combined 
digram-rating models, LR increases by a measly 1.6\%. 
% (Note that depicted LRs refer to the accuracy  of the final match(The ratio of matches that are correct).

All in all, techniques in Sections \ref{sec:kl-method} and \ref{sec:method-kl-combine} coupled 
with $Match\_All()$ yield LR of $72.2\%$ for the unigram distribution. LR goes up to $77\%$ if 
we also use ratings, and almost up to  $100\%$ if we mix in digrams. This suggests that 
our (admittedly simple) techniques are very useful in measuring privacy.


\subsection{Study Summary}
\label{sec:summary-analysis}
%
We now summarize the findings and conclusions of the study.
%
\begin{enumerate}
%
\item LRs become very high -- reaching up to $\sim$ 98\%/96\% (in KLD and NB, respectively) for record sizes of 
130/100 when we combine digrams and ratings tokens.  (See Section \ref{sec-results-digram-rate-combine}). 
With $Match\_All$, we can improve LRs to $99.4\%$, 
which includes almost all reviewers in the set. (See Section \ref{sec:inter-model}). 
%
\item Even with small record sizes, we accurately link a significant ratio of anonymous records. Specifically, for AR size of 10, 
(using NB with diagrams and ratings) we can link $76\%$ of ARs with $90\%$ of them in Top-10. This represents a significant stride 
towards linking reviewer identities. Additionally, for AR size of 50, using the same model, LR jumps to 95\% with 98\% in Top-10.
(See Section \ref{sec-results-digram-rate-combine}).   
%
\item Surprisingly, using only unigram distributions, we can link $66\%$ in both NB and KLD models, with $87\%$ in Top-10.
(See Section \ref{sec:unigram-results}). This suggests that reviewers expose a great deal merely from their single letter distributions. 
%
\item Rating is useful in tandem with lexical tokens, especially, the unigram: we witness 
a $\sim$6-7\%/5-8\% LR increase in NB/KLD for most of the record sizes. 
(See Section \ref{sec-results-uni-rate-combine}). 
%
\item Linking all anonymous records at once (instead of each one independently) helps improve accuracy.
% by leveraging the fact that every anonymous record maps to a different reviewer. 
The gain ranges from 1.6\% to 4.8\%, depending on the specific combination of tokens. (See Section \ref{sec-results-once}).   
%
\item Using rating and unigram tokens with KLD results in higher Top-1 LR: from 66.4\% (unigram only) to 72.2\%
 (unigram and rating) and up to 77\% (using $Match\_All$). (See Section \ref{sec:inter-model}). 
%
\item Performance of NB and KLD is comparable for rating and unigram. For digram, NB performs better than 
KLD for smaller records sizes while KLD scores better for larger ones. 

\end{enumerate}


==> disc-futurework.tex <==
\section{Discussion and Future Work}
\label{sec:disc-futurework}
%
\if 0
In this paper, we study the traceability and linkabilty of contributor reviews. We show that a high percentage of anonymous contributor reviews perfectly link to their original authors. Although we use very simple models and very simple features set, we are able to recover a high percentage of the anonymous records. In fact, using only the alphabetical letter distributions of contributors, we are able to recover up to 66\% of anonymous records and that can be improved to 71\% in some cases. Moreover, using the bigrams we are able to recover most of the anonymous records in spite of having many contributor (around 2000)s in our set.  
\fi
%
This paper presented the results of a study of linkabilty of reviews. We showed that a high percentage 
of anonymous reviews authored by the same person are completely linkable. 
Although we used very simple models and an equally simple features set, we could link  
a high percentage of anonymous records to corresponding identified records.

We believe that results of, and techniques used in,  this study have several implications. 
First, we demonstrate the practicality of cross-referencing accounts (and reviews) among
multiple review sites. If a person contributes to two sites under two identities, it is highly 
likely that sets of reviews from these sites can be linked 
% (given that that contributor maintain his/her pattern of writing reviews on the two sites). 
This could be quite detrimental to contributors' privacy especially, 

The second implication is the ability to correlate -- on the same review site -- multiple accounts 
that are in fact manipulated by the same person. 
This  could make our techniques very useful in detecting review spam \cite{opinion-spam-analysis},
a contributor authors reviews under different contributor-ids to tout (also self-promote) or besmirch some
product or service. One concrete application of our techniques by integrating them into review site's
front-end software in order to provide immediate feedback to authors indicating the degree of linkability
of their reviews. (It would then be up to to the individual to maintain or modify their reviewing 
patterns).
\if 0
% prolific users and history to recent....
While non-proflic reviewers are much more than prolific ones, we believe that a study on prolific users is still important for several reasons. First, the number of prolific users is large. For example, from only one user review site, we are able to collect $\sim$ 2,000 of such reviewers. Second, given the spike of the number of reviews and reviewers that some user review sites are experiencing\cite{yelpstat}, it is very conceivable that in the foreseeable future to have the user review contribution a common practice for more users and that may lead to an increasing number of review-productive users. Therefore, our study is relevant to many users and will probably be relevant to even more users in the future. 
%Finally, we believe that the problem of recovering the identities of anonymous reviews, where the contribution of each user is very limited, can not easily scale with large number of users. Thus, having prolifc users help us study the problem at a larg scale of users. 
%Thus, our study is relevant to many users and will probably be relevant to even more users in the future. 
\fi
Although our results point at high linkability of reviews among prolific contributors, there remain many open 
questions. First, it is unclear how to assess the degree of linkability if there is a small number of reviews per
author. Second, although we leverage ratings to boost the linkability ratio, we need to study the effect of using 
categories of places, products and services reviewed. We suspect that this would increase the linkability ratio 
even with a limited number of reviews. In fact, it would be interesting to see how the linkability ratio can be improved
without resorting to lexical features. (Since lexical features generally entail heavy processing and large sets of features.) 
Third, we need to investigate the linkability ratio in other preference databases (such as music/song ratings) 
and check whether contributors inadvertently link their reviews through preferences. 
\if 0
Our probelm is linking recent reviews to old ones. Although we build models that have high linkability results, we plan to more leverage the temporal effect in the reviews. There might be somehow a temporal pattern emmbedded in the reviews. For example, a user may repeat his/her choice of categories, user of words, or even the rating over different temporal episodes. As part of our future work, we plan to further study this factor and how much we can leverage it for better identifiability results. 
\fi 
As discussed in Section \ref{sec:related}, some prior studies also focused on authorship analysis. 
However, we believe that our work differs in two aspects. 

{\bf First}, we consider extensive authorship analysis in a 
different context -- user reviews. The way a person composes reviews is different from email messages, research papers,
and many other forms of writing. In a review, the contributor generally evaluates something; as a result, the text 
conveys some assessments and opinions of the contributor. A review might contain some information about the contributor's 
taste, since many contributors tend to review places, products or services that are of interest to them. In addition, reviews 
include other non-textual information, e.g.,  the rating and the category of what is being reviewed. This information gives us 
extra leverage; indeed, this paper showed the utility of using rating to increase the overall linkability ratio. 

{\bf Second}, our problem formulation is different: we focus on linking contributor identities whenever there is 
a large number of prolific contributors and one or more anonymous reviews (up to 165 reviews). Whereas, most previous related work tries to recover contributor identities
from a small set of possible authors with a small set of contributor texts and mostly, one anonymous document/message to be recovered.


==> related-longer.tex <==
\section{Related Work}
\label{sec:related}
%
Many authorship analysis studies have appeared in the literature. Among the most prominent
recent studies are: \cite{unified-data-mine, writeprints-abbasi, author-ident-framework-rong}. The study in \cite{unified-data-mine} proposes
techniques that are relied on extracting frequent pattern write-prints that characterized one (or a group of)
authors. The best achieved accuracy was 88\% when identifying an author, from a single anonymous message,
from a small set of four and with training set size of forty messages per author.



Many authorship analysis studies have appeared in the literature. Among the most prominent 
recent studies are: \cite{unified-data-mine, writeprints-abbasi, author-ident-framework-rong}. 
The study in \cite{unified-data-mine} was based on frequent pattern write-prints. It 
demonstrated some data-mining techniques that successfully identify authors from their text 
messages when either large or small training sets were used. In addition, another technique was 
presented that characterized text message authors (e.g., Gender, Age, Ethnicity). All proposed
techniques relied on extracting frequent pattern write-prints that characterized one (or a group of) 
authors. The best achieved accuracy was 88\% when identifying an author, from a single anonymous message, 
from a small set of four and with training set size of forty messages per author. 

The work in \cite{writeprints-abbasi} also considered author identification and similarity detection by incorporating 
a rich set of stylistic features along with a novel technique to extract write-prints. This technique was based 
on Karhunen-Loeve-transforms with sliding window and pattern disruption to better capture author write-prints. 
It was shown to perform well and reached as high as 91\% in identifying the author of anonymous text from a set of 100. The
same approach was tested on a large set of Buyer/Seller Ebay feedback comments collected from Ebay. 
Such comments typically reflect one's experience when dealing with a buyer or a seller. Unlike our general-purpose
reviews, these comments do not review products, services or places of different categories. Additionally, 
the scale of the problem was different and the analysis was performed for 100 authors, whereas,  our analysis
involved $\sim~2,000$ reviewers.   

In \cite{author-ident-framework-rong}, a framework for author identification for on-line messages was introduced. 
For each message, four types of features were extracted: lexical, syntactic, structural and content-specific. 
Three types of classifiers were used for author identification: Decision Trees, Back Propagation Neural Networks and 
Support Vector machines. The last one outperformed the others achieving 97\% in a set of authors that did not exceed 20.

A problem very similar to ours was explored in \cite{herbert-deanonymizer}. It focused on identifying authors 
based on reviews in both single- and double-blinded peer-reviewing processes. Na\"ive Bayes classifier was
used -- along with unigrams, bigrams and trigrams -- to identify authors. The best result was  around 90\%. In \cite{blind-review}, citations of a given paper were used to identify its authors. The data set was a very large archive of physics research papers (KDDCUP 2003 physics-paper archive). Authors were identified 40-45\% of the times.  
\if 0
In \cite{blind-review}, citations of a given paper were used to identify its authors. The data set was a very large archive 
of physics research papers (KDDCUP 2003 physics-paper archive). Two approaches were used. In one, each paper
was represented as a vector of citations  and every author was represented as the sum of the vectors of 
one's own papers. Different weighing schemes were used to weigh the vectors: binary, citation count and decayed counts
(lower weights to older papers) schemes. The closest vector in terms of cosine similarities was declared as the 
author of an anonymous paper. Accuracy reached as high as 26\% (authors exactly identified). The second approach
was very simple, yet quite effective. It simply flagged the person most cited in a given paper as its author. 
This technique correctly identified nearly 40\% of all authors.
\fi

In \cite{ngram-bayes-topic-fixed}, authorship analysis was performed on a set of candidate authors who wrote on 
the same topics. Specifically, analysis was done on movie reviews of five reviewers on the same five movies. 
Although reviews similar to ours were used, there were significant differences. We use over $1,000,000$ reviews 
by $\sim~2,000$ authors, whereas, only 25 reviews by 5 authors were used in \cite{ngram-bayes-topic-fixed}.

A related result \cite{gender-movie} studied the problem of inferring the gender of a movie reviewer from 
his/her review. Using logistic regression \cite{log-regress} along with features derived from the writing style, 
content, and meta-data of the review, accuracy of up to 73.7\% was achieved in determining correct gender.  
The goal of this study was clearly quite different from ours. For a comprehensive overview of 
authorship analysis studies, we refer to \cite{author-survey}.

While all aforementioned results are somewhat similar to our present work, there are some notable 
differences. First, we perform authorship identification analysis in a context that has not been extensively 
explored -- user reviews. User reviews are generally written differently
from other types of writing, such as email and research papers. In a review, the author generally assesses something 
and thus the text conveys some evaluation and personal opinions. A review usually conveys information about personal 
taste, since most people tend to review things of interest to them. In addition, reviews contain other non-textual information,
such as the ratings and categories of things being reviewed. These types of extra information provide added leverage; recall that,
as discussed in previous sections,  ratings are particularly helpful in increasing the overall linkability ratio. Second, our 
problem formulation is different. We study linkability of reviews (and user-ids of their authors) in the presence 
of a large number of 
prolific contributors where the number of anonymous reviews could be more than one (up to 165 reviews). Whereas, most 
prior work attempts to identify authors from a small set of authors, each with small sets of
texts where the number of anonymous documents/messages is one.       

\if 0
As discussed in Section \ref{sec:related}, some prior studies also focused on authorship identification.
However, we believe that our work differs in two aspects:

{\bf First}, we consider extensive authorship identification analysis in a unique
context of reviews. The way a person composes reviews is different from email messages, research papers,
and many other forms of writing. In a review, the contributor generally evaluates something; as a result, the text
conveys some assessments and opinions of the contributor. A review might contain some information about the contributor's
taste, since many contributors tend to review places, products or services that are of interest to them. In addition, reviews
include other non-textual information, e.g.,  the rating and the category of what is being reviewed. This information gives us
extra leverage; indeed, this paper showed the utility of using rating to increase the overall linkability ratio.

{\bf Second}, our problem formulation is distinct: we focus on linking contributor identities whenever there is
a large number of prolific contributors and one or more anonymous reviews (up to 165). Whereas, most relevant
prior work seeks to recover contributor identities from a small set of possible authors within a small set of
contributor texts. % and mostly, one anonymous document/message to be recovered.
\fi


Some work has been done in recovering authors based on their ratings, using external knowledge. In particular, 
\cite{you-what-u-say} studied author linkability with two different databases; one public and the other -- private. 
Several techniques were used to link authors in public forums (public) who state their opinions and rating  
about movies to reviewers who contribute to a sparse database (private) of movie ratings. In addition, this work
explored several measures to minimize the possibility of linking users. The study showed that authors' identities 
were generally recoverable from public databases. It also asserted the impracticality of hiding authorship data to 
protect privacy. 
However, the use of misdirection techniques (mentioning items in the public forums that a person has not rated in 
the movie rating database) helped enhance privacy and complicated linkability. A related result
\cite{deanonymize-netflix} considered
anonymity in high-dimensional and sparse data sets of anonymized users. First, it presented a general definition and model
of privacy breaches in such sets. These definitions were based on the success probability of de-anonymizing a 
specific target and on the amount of information recovered about the target. Second, a statistical de-anonymization attack 
was presented that was resilient to perturbation. Third, this attack was used to de-anonymize the Netflix \cite{netflix} 
data set. Specifically, the IMDB \cite{imdb} database was used as background knowledge and Netflix records of known 
reviewers were correctly identified. Note that the problem formulation of these two results differs from ours. 
They studied anonymity in the presence of an external source of public information. Whereas,
our work does not rely on any external sources.  

Last but not least, another related effort was made to assess the authenticity of reviews \cite{opinion-spam-analysis}. It
explored the problem of identifying spam reviews. Results demonstrated that spam reviews were 
prevalent and a counter-measure based on logistic regression was proposed. 





